4DRecons: 4D Neural Implicit Deformable Objects Reconstruction from a single RGB-D Camera with Geometrical and Topological Regularizations

This paper presents a novel approach 4DRecons that takes a single camera RGB-D sequence of a dynamic subject as input and outputs a complete textured deforming 3D model over time. 4DRecons encodes the output as a 4D neural implicit surface and presents an optimization procedure that combines a data term and two regularization terms. The data term fits the 4D implicit surface to the input partial observations. We address fundamental challenges in fitting a complete implicit surface to partial observations. The first regularization term enforces that the deformation among adjacent frames is as rigid as possible (ARAP). To this end, we introduce a novel approach to compute correspondences between adjacent textured implicit surfaces, which are used to define the ARAP regularization term. The second regularization term enforces that the topology of the underlying object remains fixed over time. This regularization is critical for avoiding self-intersections that are typical in implicit-based reconstructions. We have evaluated the performance of 4DRecons on a variety of datasets. Experimental results show that 4DRecons can handle large deformations and complex inter-part interactions and outperform state-of-the-art approaches considerably.

==> 04-4-Architecture.tex <==
\subsection{Network Architecture}
\label{Subsec:Architecture}
% where $\gamma = \big(\text{sin}(2^0\pi \bs{x}), \text{cos}(2^0\pi \bs{x}), \dots, \text{sin}(2^{L-1}\pi \bs{x}), \text{cos}(2^{L-1}\pi \bs{x}) \big) $

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.85\columnwidth]{images/network.jpg}
% \caption{Illustration of the network architecture.}
% \label{Figure:4DRecons:Architecture}
% \vspace{-0.2in}
% \end{figure}
% We implement our 4D implicit field $\bs{f}^{\theta}:\R^3 \times \R \rightarrow \R\times \R^3$ by combining a geometry branch $s^{\theta}:\R^3 \times \R \rightarrow \R^{1+f_g}$ and a color branch $c^{\theta}:\R^3 \times \R \times \R^{f_g} \rightarrow \R^{3}$. The two branches share a feature module. We also employ positional encoding to capture shape and texture details. As shown in Figure \ref{Figure:4DRecons:Architecture}, both branches employ an encoder and multilayer perceptrons (MLP). Specifically, the geometry branch $s^{\theta}$ exploits the positional encoding of the 3D coordinate $\bs{x}$ to derive a positional feature $\bs{g}_{p}$. We then feed the concatenation of $\bs{g}_{p}$ and the frame index $t$ into $8$ fully connected layers (with \textrm{softplus} activations and $512$ channels per layer) to decode the implicit value $s^{\theta}(\bs{x},t)$ and a latent feature vector $\bs{g}_{f} \in \R^{f_g}$ ($f_g = 256$). The color field utilizes multiresolution hash encoding for the 3D coordinate $\bs{x}$ and $t$ to obtain a color feature $\bs{g}_{c}$. We then feed $\bs{g}_{f}$ and $\bs{g}_{c}$ into three fully connected layers (using \textrm{ReLU} activations) to generate color $\bs{c}^{\theta}(\bs{x},t)$. Note that $\bs{g}_{p}$ encodes the correlation between the geometry branch and the color branch. 


% We implement our 4D implicit field $\bs{f}^{\theta}:\R^3 \times \R \rightarrow \R\times \R^3$ by combining a geometry branch $s^{\theta}:\R^3 \times \R \rightarrow \R^{1+f_g}$ and a color branch $c^{\theta}:\R^3 \times \R \times \R^{f_g} \rightarrow \R^{3}$. As shown in Figure~\ref{Figure:4DRecons:Architecture}, the two branches share a feature module. We also employ positional encodings to capture shape and texture details. Due to the space constraints, we defer the details to the supp. material.

We implement our 4D implicit field $\bs{f}^{\theta}:\R^3 \times \R \rightarrow \R\times \R^3$ by combining a geometry branch $s^{\theta}:\R^3 \times \R \rightarrow \R^{1+f_g}$ and a color branch $c^{\theta}:\R^3 \times \R \times \R^{f_g} \rightarrow \R^{3}$. As shown in Figure~\ref{Figure:4DRecons:Architecture}, the two branches share a feature module. We also employ positional encodings to capture shape and texture details. Due to the space constraints, we defer the details to the supp. material.
